A Smoothed Analysis of the Greedy Algorithm for the Linear Contextual Bandit Problem

Bandit learning is characterized by the tension between long-term exploration and short-term exploitation. However, as has recently been noted, in settings in which the choices of the learning algorithm correspond to important decisions about individual people (such as criminal recidivism prediction, lending, and sequential drug trials), exploration corresponds to explicitly sacrificing the well-being of one individual for the potential future benefit of others. This raises a fairness concern. In such settings, one might like to run a "greedy" algorithm, which always makes the (myopically) optimal decision for the individuals at hand - but doing this can result in a catastrophic failure to learn. In this paper, we consider the linear contextual bandit problem and revisit the performance of the greedy algorithm. We give a smoothed analysis, showing that even when contexts may be chosen by an adversary, small perturbations of the adversary's choices suffice for the algorithm to achieve "no regret", perhaps (depending on the specifics of the setting) with a constant amount of initial training data. This suggests that "generically" (i.e. in slightly perturbed environments), exploration and exploitation need not be in conflict in the linear setting.

==> alg.tex <==
\section{Perturbation Algorithm}



==> lb-new.tex <==
\section{Lower Bound: Warm start must be \jm{fill in} for sublinear regret}
\jm{under construction}
We now show that if the warm start given to greedy does not scale
polynomially with $\frac{1}{\sigma}$, the perturbation parameter, then
it can suffer linear regret.

\begin{theorem}\label{thm:lower}
  Suppose greedy is given a warm start of size $n$ for a
  $\sigma$-perturbed instance. Then, for any $R$, if
  $n = o\left(\frac{1}{\sigma^2\ln R}\right) $, then greedy will have
  regret $\Omega( \frac{R}{\sqrt{n}} )$ with constant probability over
  its first $R$ rounds.
\end{theorem}

\begin{remark}
Theorem~\ref{thm:lower} implies that, for $T < \exp(\frac{1}{\sigma})$, either
  \begin{itemize}
  \item $n$ must grow polynomially with $\frac{1}{\sigma}$, or
  \item Greedy suffers linear regret
    \end{itemize}
  \end{remark}

  We prove this theorem in the one-dimensional setting, by showing a
  warm start of size $n$ will give estimates of coefficients which
  will be too large (or too small) by an additive
  $\Omega(\frac{1}{\sqrt{n}})$ with constant probability
  (Lemma~\ref{lem:variance-ols}). If this is the case, and two arms
  have equal true coefficients, then greedy will make the wrong choice
  for contexts which are within this margin of error.  In each such
  round, greedy might incur regret $\Omega(\frac{1}{\sqrt{n}})$. So,
  it suffices to show that greedy can make a linear number of such
  mistakes.

  
  We then show that as the arms are pulled, there will be very few
  rounds (roughly $O(n^{2/3})$) for which the overestimated
  coefficient will become much smaller than its expectation
  (Lemma~\ref{lem:big-no-drift}). This will imply that for the
  underestimated arm to be pulled in $\Omega(T)$ rounds, the OLS
  estimate after one of these $O(n^{2/3})$ rounds must increase be a
  substantial amount. We show there is constant probability that this
  does not happen, so the underestimated arm is pulled at most
  $O(n^{2/3})$ round in expectation. Thus, with constant probability
  the regret of the algorithm is
  $\Omega\left({T - n^{2/3}}{\sqrt{n}}\right)$.

  We now formalize our lemmas before proving the main theorem. The
  first lemma states that the warm start of size $n$ has constant
  probability of producing OLS estimators with error on the order of
  $\frac{c_i}{\sqrt{n}}$ for any constant $c_i$.

  \begin{lemma}\label{lem:variance-ols}

    Supppose $\uxit{i}{t} = d_i \in [.5, 1]$ for all $t$ and
    $\sigma < \frac{1}{\sqrt{\ln\frac{2}{\delta}}}$.
  Further suppose
  that $\yit{i}{t}\sim \mathcal{N}(\bi{i}\pxit{i}{t}, 1)$.
  
  Then, for any constants $c_1, c_2$, with constant probability, the OLS estimators
  $\bhit{1}{}, \bhit{2}{}$ for $n$ i.i.d. samples
  $(\pxit{1}{1}, \yit{1}{1}), \ldots, (\pxit{1}{n}, \yit{1}{n})$ and
  $(\pxit{2}{1}, \yit{2}{1}), \ldots, (\pxit{2}{n}, \yit{2}{n})$ will be such that
  $\bhit{1}{} \leq \bi{1} - \frac{c_1}{\sqrt{n}}$ and
  $\bhit{2}{} \geq \bi{2}+ \frac{c_2}{\sqrt{n}}$.
\end{lemma}

The next lemma formalizes the idea that, conditioned on an initially
too-large OLS estimate, there are relatively few rounds for which that
evolving OLS estimator will be much below its expectation.

  \begin{lemma}\label{lem:big-no-drift}
  Suppose $\tfrac{T}{\delta} < 2^{n^{1/3}}$ and
    $\sigma < \frac{1}{100\sqrt{\ln \frac{T}{\delta}}}$.  Condition on the event that
    $\bhit{i}{} \geq \bi{i} + \frac{c_i}{\sqrt{n}}$ after a warm start
    of size $n$. 
    

    Then, of the $T$ rounds in which arm $i$ is pulled, 
    the expected number of rounds $t$ for
    which
    $\bhit{i}{t}\leq \bi{i} - \frac{2}{\sqrt{n}}$ is at most $0.00048 n ^{2/3}$.
   \end{lemma}



    We now proceed with the proof of Theorem~\ref{thm:lower}.
\begin{proof}[Proof of Theorem~\ref{thm:lower}]
  Consider the instance $\bi{1} = \bi{2}= 1$, and
  $\uxit{1}{t} = 1$, $\uxit{2}{t} = 1 - \frac{1}{\sqrt{n}}$ for all
  $t$, and its $\sigma$-perturbation to generate $\pxit{1}{t}, \pxit{2}{t}$.  By
  Lemma~\ref{lem:variance-ols}, for a warm start of size $n$, we will
  have $\bhit{1}{} \leq 1 - \frac{c_1}{\sqrt{n}}$ and
  $\bhit{2}{} \geq 1+\frac{c_2}{\sqrt{n}}$ with constant
  probability for any constants $c_1, c_2$. Condition on this event
  for the remainder of the proof.

  We now argue that over $T$ rounds with this initialization, there is
  constant probability that arm $1$ is pulled $o(n^{1/4})$ times while
  for $\Omega(T)$ rounds,
  $\bi{1} \pxit{1}{t} \geq \bi{2}\pxit{2}{t} - \frac{c_3}{\sqrt{n}}$. This
  implies that the for $\Omega(T - n^{1/4})$ rounds, the algorithm
  incurs regret of the order $\Omega(\frac{1}{\sqrt{n}})$.  We will
  calculate the expected number of pulls of arm $1$ conditioned on
  initialization of these estimators satisfying these inequalities. By
  Markov's inequality, it suffices to show this expectation is at most
  $m$ to show arm $1$ is pulled at most $m$ times with probability at
  least $\frac{1}{2}$. This is upper-bounded (via a union bound) by
\begin{align}\sum_{t = 1}^T \Pr{}{\textrm{arm 1 is pulled in round $t$}| \bhit{1}{} \leq 1 - \frac{c_1}{\sqrt{n}} \textrm{ and }
  \bhit{2}{} \geq 1+\frac{c_2}{\sqrt{n}}}\label{eqn:onepull}
 \end{align}

 So, we will calculate the probability arm $1$ is pulled in any round
 $t$. Consider the random perturbation of each context.  By an
 application of Hoeffding's inequality for subgaussian random
 variables (and a union bound over $2T$ events), with probability at
 least $1-\delta$, for all $t\in [T]$, we have that
 $\pxit{1}{t} \in [1 - \sigma \sqrt{2 \ln\frac{T}{\delta}}, 1 + \sigma
 \sqrt{2 \ln\frac{T}{\delta}}]$ and
 $\pxit{2}{t} \in  [1 -\frac{1}{\sqrt{n}} - \sigma \sqrt{2
   \ln\frac{T}{\delta}}, 1 -\frac{1}{\sqrt{n}} + \sigma \sqrt{2
   \ln\frac{T}{\delta}}]$. Since
 $\sigma \leq \frac{1}{10 \sqrt{2n\ln(T/\delta)}}$, then this means
 that
 $\pxit{1}{t} \in [1 - \frac{1}{10 \sqrt{n}}, 1 + \frac{1}{10 \sqrt{n}}]$
 and $\pxit{2}{t} \in [1-\frac{1.1}{\sqrt{n}},1-\frac{0.9}{\sqrt{n}}]$.
 Then, in any round $t$ such that these upper and lower bounds hold
 for $\pxit{1}{t}, \pxit{2}{t}$, arm $2$ will be pulled if
 $\bhit{2}{t} \geq 1- \frac{2}{\sqrt{n}}$ and
 $ \bhit{1}{t} \leq 1 - \frac{4}{\sqrt{n}}$, as
%
\[\bhit{2}{t}  \pxit{2}{t}\geq \left(1- \frac{2}{\sqrt{n}}\right)\left(1-\frac{1.1}{\sqrt{n}}\right)  \geq 1 - \frac{3.1}{\sqrt{n}} \geq \left(  1 - \frac{4}{\sqrt{n}}\right)\left(1 + \frac{1}{10 \sqrt{n}}\right)\geq \bhit{1}{t} \pxit{1}{t}.\]
%%%%%

So, we will upper-bound the number of rounds for which either
$\bhit{2}{t} \leq 1- \frac{2}{\sqrt{n}}$ or
$ \bhit{1}{t} \geq 1 - \frac{4}{\sqrt{n}}$ to upper-bound the
term~\ref{eqn:onepull}. Initially,
$\bhit{1}{} \leq 1 - \frac{4}{\sqrt{n}}$ for an appropriate
$c_1$. Lemma~\ref{lem:big-no-drift} imples that there are at most
$0.00048n^{2/3}$ rounds after which arm $2$ is pulled for which
$\bhit{2}{t} \leq 1- \frac{2}{\sqrt{n}}$. We now argue that there is
constant probability that none of these following rounds (in which arm
$1$ might be pulled) causes arm $1$'s estimate to be large, i.e.  that
$ \bhit{1}{t} \leq 1 - \frac{4}{\sqrt{n}}$ for all rounds $t$ with
constant probability, and therefore that arm $1$ is pulled at most
$0.00048n^{2/3}$ times with constant probability.

We now upper bound the probability than any one of these pulls
of arm $1$ causes $\bhit{1}{t} \geq 1 - \frac{4}{\sqrt{n}}$ when
$\bhit{1}{} \leq 1-\frac{c_1}{\sqrt{n}}$.  This initial underestimate implies that
$\sum_{i=1}^n \pxit{1}{t} \nit{1}{t} \leq \frac{- c_1\sqrt{n}}{2}$, using the
lower bound on $\pxit{2}{t}$. The noise component of $\bhit{1}{t}$ for rounds $t$ before
its OLS estimator has ever been  small 
is then

\begin{align*}
\bhit{1}{t} - \bi{1} & =   \frac{\sum_{i = 1}^n \pxit{1}{t} \nit{1}{t}  + \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} \pxit{1}{t'} \nit{1}{t'}}{\sum_{i = 1}^n (\pxit{1}{t})^2 +  \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} (\pxit{1}{t'})^2}\\
  & \leq  \frac{ \frac{- c_1\sqrt{n}}{2}  + \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} \pxit{1}{t'} \nit{1}{t'}}{\sum_{i = 1}^n (\pxit{1}{t})^2 +  \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} (\pxit{1}{t'})^2}\\
  & \leq  \frac{ \frac{- c_1\sqrt{n}}{2}  + \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} \pxit{1}{t'} \nit{1}{t'}}{.8 n   }\\
  & \leq  \frac{ \frac{- c_1\sqrt{n}}{2}  + \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} \pxit{1}{t'} \nit{1}{t'}}{.8 n }\\
  &  \leq \frac{- 5c_1}{8\sqrt{n}}  +  \frac{ \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}} \pxit{1}{t'} \nit{1}{t'}}{.8 n }\\
  & = \frac{- 5c_1}{8\sqrt{n}}  + \sum_{  t' : \textrm{ arm 1 pulled because $\bhit{2}{t} \leq 1-\frac{2}{\sqrt{n}}$}}   \frac{1.01}{.8n} \nit{1}{t'}\\
  & \leq \frac{- 5c_1}{8\sqrt{n}}  +   \frac{1.3}{n} \sqrt{2 \cdot 0.00048n^{2/3} \ln  \frac{00048n^{2/3} }{\delta}}\\
    & \leq \frac{- 5c_1}{8\sqrt{n}}  +   \frac{1.3}{n^{2/3}} \sqrt{2 \cdot 0.00048 \ln  \frac{00048n^{2/3} }{\delta}}\\
\end{align*}
%
where the second to last inequality holds with probability $1-\delta$
(for all of these $.00048n^{2/3}$ rounds by a Hoeffding bound for
Gaussians). Finally, we note that this term is less than
$ \frac{-4}{\sqrt{n}}$ for properly chosen constants $c_1, \delta$ and
for superconstant $n$. Thus, with constant probability,
$\bhit{1}{t} < 1 - \frac{4}{\sqrt{n}}$ for all rounds $t$, and for
all but $0.00048 n^{2/3}$ rounds,
$\bhit{2}{t} \geq 1 - \frac{2}{\sqrt{n}}$, therefore implying arm
$2$ will be pulled all but $0.00048 n^{2/3}$ rounds with constant
probability. Each round has constant probability that the regret from
pulling arm $2$ rather than arm $1$ is $\Omega(\frac{1}{\sqrt{n}})$,
and so the regret is $\Omega(\frac{T}{\sqrt{n}})$ with constant
probability.
\end{proof}


\begin{proof}
  Consider $\uxit{i}{t} = 1$ and $\bi{1} = 2\epsilon $ while
  $\bi{2}=  \epsilon $. Lemma~\ref{lem:variance-ols} implies there's
  constant probability that
  $\bhit{1}{} \leq 2\epsilon - \frac{c_1}{\sqrt{n}}, \bhit{2}{} \geq 
  \epsilon + \frac{c_2}{\sqrt{n}}$ for the initial OLS estimators
  after a warm start of size $n$. If $\frac{1}{\sqrt{n}} > \epsilon$,
  this implies with constant probability that
  $\bhit{1}{} \leq  (1 - c_1 )\epsilon \leq \epsilon$ and
  $\bhit{2}{} \geq (c_2 - 1)\epsilon \geq 2\epsilon$ for
  $ c_1, c_2 \geq 2$.

  So, initially, our estimates will cause us to pull arm $2$ rather
  than arm $1$ for most contexts. We now calculate the expected number
  of rounds before we will pull arm $1$ (over the randomness of the
  perturbed contexts), before this point $\bhit{1}{t}=
  \bhit{1}{}$. So, we calculate the expected number of rounds for
  which the following holds.
  
  \[\bhit{2}{t} \pxit{2}{t}   \geq \bhit{1}{t} \pxit{1}{t} = \bhit{1}{} \pxit{1}{t}\]

  If we assume ${\sigma} < \frac{1}{100\sqrt{\ln\frac{T}{\delta}}}$,
  then with probability $1-\delta$, it is the case that
  $\pxit{i}{t} \in [.99, 1.01]$ for all $i\in \{1,2\}, t\in [T]$ by a
  union bound and Chernoff for Gaussian random variables.  So, to
  bound the expected number of rounds $t$ for which the previous
  inequality holds, it suffices to consider the rounds $t$ for which
  $\bhit{2}{t} \geq -\frac{\epsilon}{3}$ and
  $\bhit{1}{t} \leq \frac{-\epsilon}{2}$

  
  \end{proof}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> smooth.tex <==
\section{Smoothed Analysis} \label{sec:smooth}

\subsection{Some Lemmas}


\subsection{Single-Parameter}


\subsection{Multiple-Parameter}


